Towards On-device Learning on the Edge: Ways to Select Neurons to Update under a Budget Constraint

In the realm of efficient on-device learning under extreme memory and computation constraints, a significant gap in successful approaches persists. Although considerable effort has been devoted to efficient inference, the main obstacle to efficient learning is the prohibitive cost of backpropagation. The resources required to compute gradients and update network parameters often exceed the limits of tightly constrained memory budgets. This paper challenges conventional wisdom and proposes a series of experiments that reveal the existence of superior sub-networks. Furthermore, we hint at the potential for substantial gains through a dynamic neuron selection strategy when fine-tuning a target task. Our efforts extend to the adaptation of a recent dynamic neuron selection strategy pioneered by Bragagnolo et al. (NEq), revealing its effectiveness in the most stringent scenarios. Our experiments demonstrate, in the average case, the superiority of a NEq-inspired approach over a random selection. This observation prompts a compelling avenue for further exploration in the area, highlighting the opportunity to design a new class of algorithms designed to facilitate parameter update selection. Our findings usher in a new era of possibilities in the field of on-device learning under extreme constraints and encourage the pursuit of innovative strategies for efficient, resource-friendly model fine-tuning.

==> Tables/baselines.tex <==
\begin{table*}[hbt!]
\caption{Full networks fine-tuning on various image classification datasets.}
\centering
\renewcommand*{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\label{tab:results:baselines}
    \begin{tabular}{ccccccccc}
        \toprule
        \textbf{ } & $\bf \mathcal{B}^w$ & \textbf{Cifar 10} & \textbf{Cifar 100} & \textbf{VWW} & \textbf{Flowers} & \textbf{Food} & \textbf{Pets} & \textbf{CUB} \\
        \midrule
        Mbv2 & 2 189 760 & 93.47\small$\pm$0.09 & 74.51\small$\pm$0.43 & \textbf{87.47\small$\pm$0.05} & 73.05\small$\pm$1.03 & 76.69\small$\pm$0.23 & 70.15\small$\pm$0.10 & 52.06\small$\pm$0.40 \\

        \midrule

        Resnet18 & 11 166 912 & 94.00\small$\pm$0.15 & 74.61\small$\pm$0.23 & 85.98\small$\pm$0.26 & \textbf{73.58\small$\pm$0.45} & 73.58\small$\pm$0.16 & \textbf{69.75\small$\pm$0.83} & 51.46\small$\pm$0.33 \\

        \midrule
        
        Resnet50 & 23 454 912 & \textbf{94.68\small$\pm$0.08} & \textbf{76.04\small$\pm$0.55} & 87.04\small$\pm$0.20 & 70.53\small$\pm$0.83 & \textbf{76.87\small$\pm$0.14} & 68.88\small$\pm$1.04 & \textbf{52.91\small$\pm$0.59} \\
        \bottomrule
    \end{tabular}
}
\end{table*}
